Tunable coupling scheme for implementing two-qubit gates on fluxonium qubits

The superconducting fluxonium circuit is an RF-SQUID-type flux qubit that uses a large inductance built from an array of Josephson junctions or a high kinetic inductance material. This inductance suppresses charge sensitivity exponentially and flux sensitivity quadratically. In contrast to the transmon qubit, the anharmonicity of fluxonium can be large and positive, allowing for better separation between the low energy qubit manifold of the circuit and higher-lying excited states. Here, we propose a tunable coupling scheme for implementing two-qubit gates on fixed-frequency fluxonium qubits, biased at half flux quantum. In this system, both qubits and coupler are coupled capacitively and implemented as fluxonium circuits with an additional harmonic mode. We investigate the performance of the scheme by simulating a universal two-qubit fSim gate. In the proposed approach, we rely on a planar on-chip architecture for the whole device. Our design is compatible with existing hardware for transmon-based devices, with the additional advantage of lower qubit frequency facilitating high-precision gating.

==> bibliography.tex <==
 \citenamefont {ref. com. 1.1}]{equation 4}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Jérôme}\ \bibnamefont
  {Bourassa}}, \bibinfo {author} {\bibfnamefont {Félix}\ \bibnamefont {Beaudoin}},
  \bibinfo {author} {\bibfnamefont {Jay M.}\ \bibnamefont {Gambetta}},
  \bibinfo {author} {\bibfnamefont {A.}\ \bibnamefont {Blais}},
  \bibnamefont {Meyer}}, \bibinfo {author}
 \bibfield  {title}
  {\enquote {\bibinfo {title} {Josephson-junction-embedded transmission-line resonators: From Kerr medium to in-line transmon},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {5}},\
  \bibinfo {pages} {86} (\bibinfo {year} {2012})}\BibitemShut {NoStop}%
   \citenamefont {ref. com.1.2}]{equation 4}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {B. Peropadre}}\ \bibnamefont
  {J. Lindkvist}}, \bibinfo {author} {\bibfnamefont {I-C. Hoi}\ \bibnamefont {C. M. Wilson}},
  \bibinfo {author} {\bibfnamefont {J. J. Garcia-Ripoll}\ \bibnamefont {P. Delsing}},
  \bibinfo {author} {\bibfnamefont {G. Johanssonn}}\
 \bibfield  {title}
  {\enquote {\bibinfo {title} {Scattering of coherent states on a single artificial atom},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {New Journal of Physics}\ }\textbf {\bibinfo {volume} {15}},\ (\bibinfo {year} {2013})}\BibitemShut {NoStop}%
  \citenamefont {ref. com.1.3}]{equation 4}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Kevin Lalumière}\ \bibnamefont
  {Barry C. Sanders}}, \bibinfo {author} {\bibfnamefont {Félix}\ \bibnamefont {Beaudoin}},
  \bibinfo {author} {\bibfnamefont {Jay M.}\ \bibnamefont {A. F. van Loo}},
  \bibinfo {author} {\bibfnamefont {A. Fedorov}\ \bibnamefont { A. Wallraff}},
  \bibnamefont {A. Blais}}, \bibinfo {author}
 \bibfield  {title}
  {\enquote {\bibinfo {title} {Input-output theory for waveguide QED with an ensemble of inhomogeneous atoms},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {5}},\
  \bibinfo {pages} {88} (\bibinfo {year} {2013})}\BibitemShut {NoStop}%
  \citenamefont {ref. com.1.4}]{equation 4}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Moein Malekakhlagh}}\ \bibnamefont {Hakan E. Türeci}}
 \bibfield  {title}
  {\enquote {\bibinfo {title} {Origin and implications of an 
A^2-like contribution in the quantization of circuit-QED systems},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {5}},\
  \bibinfo {pages} {93} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
   \citenamefont {ref. com.1.5}]{equation 4}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {Henrik Lund Mortensen}\ \bibnamefont}
  {Klaus Mølmer}}, \bibinfo {author} {\bibfnamefont {Christian Kraglund Andersen}\ }
 \bibfield  {title}
  {\enquote {\bibinfo {title} {Normal modes of a superconducting transmission-line resonator with embedded lumped element circuit components},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Phys. Rev.}\ }\textbf {\bibinfo {volume} {5}},\
  \bibinfo {pages} {94} (\bibinfo {year} {2016})}\BibitemShut {NoStop}%
   \citenamefont {ref. com.1.6}]{equation 4}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {A. Parra-Rodriguez}\ \bibnamefont
  {E. Rico}}, \bibinfo {author} {\bibfnamefont {E. Solano}\ \bibnamefont {L. Egusquiza}}}
 \bibfield  {title}
  {\enquote {\bibinfo {title} {Quantum networks in divergence-free circuit QED},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Quantum Science and Technology}\ }\textbf {\bibinfo {volume} {3}},\ (\bibinfo {year} {2018})}\BibitemShut {NoStop}%
  \citenamefont {ref. com. 4}]{fig. 2}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {O. Astafiev}\ \bibnamefont
  {A. M. Zagoskin}}, \bibinfo {author} {\bibfnamefont { A. A. Abdumalikov Jr.}\ \bibnamefont {Yu. A. Pashkin}},
  \bibinfo {author} {\bibfnamefont {T. Yamamoto}\ \bibnamefont { K. Inomata}},
  \bibinfo {author} {\bibfnamefont {Y. Nakamura}\ \bibnamefont {J. S. Tsai}}}
 \bibfield  {title}
  {\enquote {\bibinfo {title} {Resonance Fluorescence of a Single Artificial Atom},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Science}\ }\textbf {\bibinfo {volume} {327}},\
  \bibinfo {pages} {840-843} (\bibinfo {year} {2010})}\BibitemShut {NoStop}%
  \citenamefont {ref. com. 7}]{ultrastrongly c.q.}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {P. Forn-Díaz}\ \bibnamefont
  {J. J. García-Ripoll}}, \bibinfo {author} {\bibfnamefont {B. Peropadre}\ \bibnamefont {J.-L. Orgiazzi}},
  \bibinfo {author} {\bibfnamefont {M. A. Yurtalan}\ \bibnamefont {R. Belyansky}},
  \bibinfo {author} {\bibfnamefont {C. M. Wilson}\ \bibnamefont { A. Lupascu}}}
 \bibfield  {title}
  {\enquote {\bibinfo {title} {Ultrastrong coupling of a single artificial atom to an electromagnetic continuum in the nonperturbative regime},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Nature Physics}\ }\textbf {\bibinfo {volume} {13}},\
  \bibinfo {pages} {39-43} (\bibinfo {year} {2017})}\BibitemShut {NoStop}%
    \citenamefont {ref. com. 8}]{Fig. 6}%
  \BibitemOpen
  \bibfield  {author} {\bibinfo {author} {\bibfnamefont {R. Vijay}\ \bibnamefont
  {M. H. Devoret}}, \bibinfo {author} {\bibfnamefont { I. Siddiqi}\}}}
 \bibfield  {title}
  {\enquote {\bibinfo {title} {Invited Review Article: The Josephson bifurcation amplifier},}\ }\href@noop {} {\bibfield  {journal} {\bibinfo
  {journal} {Review of Scientific Instruments}\ }\textbf {\bibinfo {volume} {80}},\ (\bibinfo {year} {2009})}\BibitemShut {NoStop}%
